The infrared compactness-temperature relation for quiescent and starburst galaxies

IRAS observations show the existence of a correlation between the infrared luminosity Lir and dust temperature Td in star-forming galaxies, in which larger Lir leads to higher dust temperature. The Lir-Td relation is commonly seen as reflecting the increase in dust temperature in galaxies with higher star formation rate. Even though the correlation shows a significant amount of dispersion, a unique relation has been commonly used to construct spectral energy distributions of galaxies in distant universe studies, such as source number counting or photometric redshift determination. In this work, we introduce a new parameter, namely the size of the star-forming region Rir and lay out the empirical and modelled relation between the global parameters Lir, Td and Rir of IR-bright non-AGN galaxies. IRAS 60-to-100um color is used as a proxy for the dust temperature and the 1.4GHz radio contiuum emission for the infrared spatial distribution. The analysis has been carried out on two samples. The first one is made of the galaxies from the 60um flux-limited IRAS Revised Bright Galaxy Samples which have a reliable RC size estimate from the VLA follow-ups of the IRAS Bright Galaxy Samples. The second is made of the sources from the 170um ISOPHOT Serendipity Sky Survey which are resolved by the NVSS or FIRST surveys. We show that the dispersion in the Lir-Td diagram can be reduced to a relation between the infrared surface brightness and the dust temperature, a relation that spans 5 orders of magnitude in surface brightness. We explored the physical processes giving rise to the Sir-Td relation, and show that it can be derived from the Schmidt law, which relates the star formation rate to the gas surface density.

==> 3881inp1.tex <==
NGC 7817         &279   &00 03 58.90&+20 45 08.4&Sbc &33.9&10.27& 0.37&3.77&1.94&29.1\\
UGC 00148        &1051  &00 15 51.26&+16 05 23.4&Sbc &  62&10.36& 0.44&3.64&2.29&32.8\\
MCG -01-01-064   &1109  &00 16 50.87&-05 16 06.1&SBa &56.8&10.29& 0.89&3.55&2.39&31.6\\
MCG +08-01-041   &1414  &00 22 01.22&+49 08 00.1&Sc  &77.7&10.44& 0.63&3.59&2.46&32.7\\
UGC 00256        &1658  &00 26 56.53&+50 01 50.4&Sbc &78.1&10.61& 1.00&3.68&2.45&31.2\\
IC 1562          &2308  &00 38 33.95&-24 16 26.8&SBc &52.6&10.00& 0.14&3.71&1.78&29.6\\
NGC 0200         &2387  &00 39 34.85&+02 53 14.7&Sbc &74.7&10.42& 0.13&3.77&2.08&30.0\\
NGC 0214         &2479  &00 41 28.01&+25 29 57.6&SABc&67.1&10.51& 0.10&3.60&2.51&29.0\\
NGC 0245         &2691  &00 46 05.39&-01 43 24.2&Sb  &58.2&10.56& 0.19&3.65&2.46&32.5\\
UGC 00540        &3108  &00 52 58.29&+29 01 56.5&Sb  &73.8&10.28& 0.29&3.65&2.18&33.9\\
MCG -05-03-011   &3159  &00 53 43.45&-27 02 59.3&Sc  &78.2&10.40& 0.62&3.63&2.35&32.4\\
NGC 0418         &4189  &01 10 35.61&-30 13 16.6&Sc  &80.2&10.48& 0.01&3.89&1.90&30.9\\
IC 1671          &4724  &01 19 02.34&-17 03 37.5&Sb  &84.8&10.81& 0.75&3.63&2.75&37.8\\
NGC 0470         &4777  &01 19 44.83&+03 24 35.8&Sb  &31.1&10.19& 0.30&3.27&2.85&36.8\\
NGC 0491         &4914  &01 21 20.43&-34 03 47.8&SBb &53.3&10.45& 0.36&3.51&2.63&29.3\\
MCG -07-04-004   &5278  &01 25 28.48&-38 16 02.4&S0-a&86.6&10.12& 0.17&3.98&1.37&29.7\\
MCG -04-06-009   &8223  &02 09 18.08&-23 24 54.2&Sbc &74.7&10.78& 0.49&3.64&2.71&29.7\\
UGC 02028        &9729  &02 33 18.19&+22 23 37.8&Sc  &79.2&10.38& 0.41&3.89&1.80&27.8\\
NGC 1070         &10309 &02 43 22.29&+04 58 06.4&Sb  &58.3&10.27&-0.14&3.72&2.05&27.8\\
UGC 02198        &10319 &02 43 32.65&+31 47 24.0&Scd &69.4&10.32& 0.96&3.76&2.01&29.6\\
NGC 1077 NED02   &10468 &02 46 00.57&+40 05 24.6&Sb  & 133&10.67& 0.22&3.88&2.11&30.5\\
NGC 1094         &10559 &02 47 27.81&-00 17 06.5&SABa&92.5&10.53& 0.15&3.89&1.96&29.2\\
NGC 1103         &10597 &02 48 05.99&-13 57 33.3&SBb &57.7&10.24& 0.23&3.78&1.88&30.9\\
UGC 02380        &11011 &02 55 11.09&+51 54 25.7&Sb  &69.7&10.10&     &3.86&1.58&29.4\\
UGC 02409        &11134 &02 56 44.98&+50 35 43.5&Sbc &58.8&10.53& 1.40&3.62&2.49&32.9\\
MRK 0602         &11336 &02 59 50.60&+02 46 16.7&SBbc&36.9&10.03& 0.51&3.26&2.71&37.7\\
UGC 02801        &13410 &03 38 19.79&+41 17 34.0&Sc  &73.8&10.23& 0.96&3.81&1.80&29.9\\
IRAS F03379+6754 &165371&03 42 46.70&+68 04 02.7&Sc  & 161&11.00& 1.37&3.89&2.42&35.0\\
UGC 03028        &15047 &04 24 35.23&+33 52 29.8&Sb  &80.5&10.68& 1.19&3.85&2.19&29.4\\
UGC 03089        &15533 &04 33 54.00&+16 54 43.5&Sbc &66.4&10.09& 0.66&3.61&2.07&29.2\\
NGC 1620         &15638 &04 36 37.34&-00 08 36.9&SABc&49.3&10.15&-0.02&3.84&1.68&28.0\\
IC 0391          &16402 &04 57 21.18&+78 11 25.3&Sc  &24.8& 9.90& 0.38&3.32&2.47&37.1\\
NGC 1843         &16949 &05 14 06.14&-10 37 36.6&SABc&  35& 9.94& 0.24&3.62&1.90&30.5\\
IRAS 05175+0547  &17126 &05 20 12.59&+05 50 15.2&Sb  & 124&10.77& 0.77&3.80&2.38&34.6\\
NGC 2076         &17804 &05 46 47.46&-16 46 57.5&S0-a&29.5&10.30& 1.00&3.42&2.66&29.5\\
UGC 03340        &17839 &05 47 27.36&+79 38 09.1&Sab &68.6&10.61& 0.92&3.61&2.60&34.2\\
ESO 055415-1941.8&18115 &05 56 25.18&-19 41 31.0&Sab &37.3& 9.93& 0.59&3.28&2.58&33.3\\
MCG -03-16-006   &18220 &06 00 20.49&-16 10 00.0&Sa  &92.6&10.66& 0.79&3.67&2.52&33.1\\
IC 0454          &19725 &06 51 06.30&+12 55 19.6&SBab&56.8&10.32&     &3.75&2.01&29.2\\
UGC 03830        &20894 &07 23 30.55&+02 36 56.8&SBcd&  20& 9.33& 0.72&3.22&2.09&33.0\\
NGC 2446         &21860 &07 48 39.26&+54 36 43.0&Sb  &85.2&10.54& 0.17&3.82&2.11&28.4\\
NGC 2958         &27620 &09 40 41.61&+11 53 18.4&SABb&97.5&10.56& 0.10&3.76&2.24&31.4\\
NGC 3218         &30323 &10 21 49.00&+74 10 36.8&SBbc&49.4&10.41& 0.16&3.65&2.30&29.6\\
MCG -06-23-029   &30716 &10 27 02.50&-36 13 41.5&Sbc &43.6&10.06& 0.62&3.63&2.01&31.2\\
MCG -05-25-031   &31677 &10 39 14.89&-30 17 52.1&Sbc &53.1&10.20& 0.36&3.52&2.35&30.8\\
NGC 3430         &32614 &10 52 11.41&+32 57 01.5&Sc  &28.7& 9.94&-0.04&3.72&1.70&30.8\\
ARP 062          &37282 &11 53 39.95&+43 27 39.6&Sab &89.3&10.67& 0.59&3.88&2.12&33.7\\
NGC 4125A        &38212 &12 04 33.92&+64 26 12.2&Sa  &26.6& 9.55& 0.08&3.32&2.12&32.6\\
NGC 4205         &39143 &12 14 55.33&+63 46 55.7&Sbc &26.2& 9.55& 0.16&3.36&2.04&32.1\\
NGC 4294         &39925 &12 21 17.81&+11 30 38.4&SBc &  18& 9.34&-0.17&3.35&1.84&33.9\\
NGC 4299         &39968 &12 21 40.52&+11 30 10.8&SABd&  18& 9.30&-0.07&3.28&1.94&34.6\\
NGC 4383         &40516 &12 25 25.53&+16 28 12.1&Sa  &15.3& 9.61& 0.38&2.88&3.06&38.9\\
NGC 4402         &40644 &12 26 07.57&+13 06 46.1&Sb  &15.3& 9.66& 0.53&3.28&2.30&28.5\\
IRAS F12334+6414 &41961 &12 35 42.04&+63 58 25.5&S?  & 163&11.04& 0.64&3.98&2.28&31.2\\
IC 3587          &42083 &12 36 48.35&+27 32 55.0&Sc  & 110&10.33& 0.63&4.22&1.09&30.5\\
MCG -03-33-003   &42954 &12 44 51.84&-20 25 35.4&Sc  &91.7&10.77& 0.38&3.69&2.59&33.2\\
NGC 4670         &42987 &12 45 17.15&+27 07 31.9&S0-a&11.8& 8.87& 0.05&2.95&2.17&37.1\\
NGC 4701         &43331 &12 49 11.55&+03 23 19.5&Sc  &  22& 9.56& 0.06&3.37&2.03&31.5\\
NGC 4868         &44557 &12 59 08.90&+37 18 36.9&Sab &71.8&10.71& 0.22&3.57&2.77&31.3\\
NGC 4900         &44797 &13 00 39.15&+02 30 05.3&SBc &15.4& 9.58& 0.04&3.31&2.17&32.0\\
NGC 4981         &45574 &13 08 48.74&-06 46 39.3&Sbc &29.9&10.02&-0.04&3.72&1.77&31.4\\
NGC 5012         &45795 &13 11 37.04&+22 54 55.5&Sc  &43.6&10.23& 0.12&3.77&1.90&30.1\\
MCG -05-31-039   &45901 &13 12 55.44&-32 41 23.5&SBcd&35.9& 9.65&-0.03&3.88&1.09&30.2\\
NGC 5056         &46180 &13 16 12.33&+30 57 01.0&Sc  &  85&10.37& 0.06&3.76&2.05&32.0\\
NGC 5113         &46589 &13 20 52.79&+57 38 29.5&Sbc &36.5& 9.51&-0.24&3.42&1.86&34.8\\
NGC 5149         &47011 &13 26 09.17&+35 56 04.0&SBbc&86.2&10.90& 0.53&3.66&2.79&34.8\\
NGC 5301         &48816 &13 46 24.61&+46 06 26.7&SBc &29.8& 9.88& 0.33&3.86&1.35&27.3\\
NGC 5303A        &48917 &13 47 44.96&+38 18 16.2&Sc  &26.9& 9.75& 0.02&3.30&2.36&33.5\\
NGC 5351         &49359 &13 53 27.72&+37 54 54.0&SBb &  57&10.12&-0.09&3.92&1.49&29.5\\
NGC 5372         &49451 &13 54 45.98&+58 39 59.0&S?  &30.8& 9.73& 0.22&3.22&2.49&34.4\\
IC 4367          &50266 &14 05 36.57&-39 12 12.2&SABc&  59&10.36& 0.15&3.74&2.08&28.2\\
NGC 5480         &50312 &14 06 21.52&+50 43 30.0&Sc  &34.4&10.13& 0.24&3.37&2.58&30.1\\
NGC 5504         &50718 &14 12 15.83&+15 50 31.2&Sbc &79.5&10.39& 0.16&3.72&2.14&30.9\\
NGC 5526 NED02   &50832 &14 13 53.73&+57 46 16.7&Sbc &34.8& 9.85& 0.73&3.26&2.54&32.2\\
NGC 5522         &50889 &14 14 50.36&+15 08 48.1&Sb  &69.8&10.40& 0.35&3.68&2.24&34.0\\
NGC 5533         &50973 &14 16 07.69&+35 20 37.5&Sab &60.7&10.18&-0.25&3.71&1.96&26.1\\
IC 0991          &51059 &14 17 48.59&-13 52 22.4&SBc &68.9&10.35& 0.25&3.88&1.79&28.8\\
NGC 5592         &51428 &14 23 55.06&-28 41 17.3&Sbc &62.8&10.58& 0.46&3.58&2.62&30.5\\
NGC 5614         &51439 &14 24 07.61&+34 51 32.1&Sab &  61&10.30&-0.18&3.66&2.17&26.7\\
NGC 5604         &51471 &14 24 42.80&-03 12 43.7&Sa  &42.8&10.18& 0.41&3.46&2.45&31.2\\
NGC 5637         &51736 &14 28 59.64&+23 11 29.5&Sc  &80.1&10.41& 0.56&3.64&2.33&32.7\\
MCG -04-34-019   &51902 &14 31 32.15&-25 23 12.1&Sc  &38.3& 9.77& 0.44&3.39&2.19&30.2\\
IC 4468          &52324 &14 38 26.79&-22 22 03.0&SBc &  37& 9.71& 0.22&3.72&1.47&28.9\\
IC 1048          &52564 &14 42 57.88&+04 53 24.6&Sbc &29.7& 9.70& 0.35&3.50&1.90&29.4\\
UGC 09509 NOTES01&52726 &14 46 01.81&+08 29 46.0&    & 156&10.83& 1.01&3.91&2.21&35.6\\
NGC 5757         &52839 &14 47 46.37&-19 04 42.8&Sb  &36.3&10.31& 0.57&3.37&2.78&35.0\\
NGC 5875         &54095 &15 09 13.21&+52 31 42.0&Sb  &56.4&10.40& 0.22&3.74&2.12&28.4\\
NGC 5908         &54522 &15 16 43.23&+55 24 33.5&Sb  &53.3&10.65& 0.39&3.86&2.13&28.2\\
NGC 5961         &55515 &15 35 16.25&+30 51 50.9&Sb  &30.7& 9.52& 0.41&3.32&2.08&34.8\\
ESO 154918-3842.1&56278 &15 52 36.60&-38 51 00.7&Sbc &65.7&10.61& 1.46&3.58&2.65&31.8\\
IC 1151          &56537 &15 58 32.31&+17 26 29.7&SBc &36.2& 9.59&-0.08&3.59&1.61&30.9\\
UGC 10123        &56570 &15 59 02.75&+51 18 16.1&Sab &  60&10.28& 0.68&3.60&2.28&29.3\\
IC 1210          &57589 &16 14 30.14&+62 32 12.0&Sab &  48& 9.93& 0.63&3.50&2.14&31.2\\
NGC 6168         &58423 &16 31 21.41&+20 11 04.8&Sd  &41.1& 9.88& 0.47&3.56&1.97&32.2\\
IC 1228          &58804 &16 42 06.50&+65 35 08.0&Sab & 116&11.07& 0.72&3.79&2.69&33.9\\
IRAS F16463-0642 &90256 &16 49 01.59&-06 47 28.0&S?  &94.1&10.67&     &3.78&2.32&34.5\\
NGC 6246A        &59090 &16 50 13.98&+55 23 04.8&Sc  &81.6&10.36& 0.23&4.09&1.39&28.6\\
MCG -01-43-002   &59133 &16 51 32.32&-03 05 46.9&Sbc & 107&10.74& 0.84&4.13&1.69&30.1\\
NGC 6368         &60315 &17 27 11.55&+11 32 32.9&Sb  &44.1&10.10& 0.18&3.62&2.06&29.1\\
NGC 6372         &60330 &17 27 31.86&+26 28 30.6&Sbc &73.3&10.42& 0.23&3.77&2.08&29.9\\
UGC 10885        &60403 &17 30 08.34&+35 21 59.3&Sb  & 122&10.75& 0.66&3.90&2.15&30.2\\
NGC 6389         &60466 &17 32 39.78&+16 24 06.2&Sbc &49.3&10.07&-0.11&3.91&1.45&29.7\\
UGC 10976        &60833 &17 46 27.83&+30 42 17.0&SBbc&75.9&10.45&     &3.71&2.24&32.0\\
NGC 6478         &60896 &17 48 38.33&+51 09 26.2&Sc  & 104&10.79& 0.34&3.89&2.22&27.8\\
IRAS F18023+2311 &165751&18 04 26.08&+23 11 20.5&S?  & 161&11.03&     &3.93&2.37&36.3\\
MCG +02-46-012   &61658 &18 15 58.28&+13 47 07.1&Sc  &47.4& 9.93& 0.47&3.52&2.09&31.2\\
IRAS 18216+5117  &61797 &18 22 50.70&+51 19 09.5&S?  & 126&10.76& 0.60&3.82&2.33&32.1\\
NGC 6632         &61849 &18 25 03.09&+27 32 07.3&Sbc &73.4&10.50& 0.02&3.98&1.74&29.9\\
NGC 6640         &61913 &18 28 08.24&+34 18 09.7&Sc  & 104&10.40& 0.29&4.00&1.60&31.7\\
NGC 6678         &61972 &18 30 39.80&+67 59 13.3&SABa&42.6&10.09& 0.26&3.34&2.62&32.7\\
NGC 6677         &62035 &18 33 36.12&+67 06 38.4&Sbc & 102&10.86& 0.37&3.75&2.57&33.4\\
NGC 6700         &62376 &18 46 04.42&+32 16 46.5&SBc &  71&10.09& 0.01&3.95&1.38&29.4\\
UGC 11379        &62593 &18 56 43.96&+25 14 13.9&Sc  &  68&10.06& 0.48&3.65&1.96&35.4\\
UGC 11404        &62781 &19 07 03.79&+29 00 23.1&Sbc &  61&10.47& 0.41&3.85&1.97&30.2\\
UGC 11428        &63084 &19 20 28.55&+30 49 31.6&SABc&61.5&10.27& 0.45&3.70&2.08&30.7\\
NGC 6796         &63121 &19 21 30.82&+61 08 41.5&Sbc &37.1&10.23& 0.56&3.51&2.42&28.9\\
NGC 6801         &63229 &19 27 35.80&+54 22 22.5&Sc  &67.5&10.32& 0.48&3.90&1.73&29.9\\
UGC 11453        &63311 &19 31 08.05&+54 06 07.8&Sb  &60.7&10.53& 0.20&3.65&2.42&29.0\\
IC 1303          &63328 &19 31 30.06&+35 52 35.8&Sc  &69.1&10.23& 0.54&3.80&1.83&30.8\\
NGC 6824         &63575 &19 43 40.65&+56 06 33.9&Sab &  49&10.62& 0.48&3.41&3.00&30.9\\
NGC 6911         &64485 &20 19 38.32&+66 43 42.2&SBb &41.4&10.29& 1.05&3.54&2.40&30.9\\
NGC 6898         &64517 &20 21 08.01&-12 21 32.3&SBa &83.2&10.59&     &3.68&2.44&31.9\\
NGC 6916         &64600 &20 23 33.06&+58 20 38.6&SBbc&49.8&10.30& 0.96&3.73&2.04&29.2\\
NGC 6928         &64932 &20 32 50.21&+09 55 35.2&SBab&70.8&10.50& 0.29&3.82&2.07&29.5\\
NGC 6949         &65010 &20 35 06.94&+64 48 10.2&Sc  &  45& 9.93& 0.50&3.65&1.84&29.0\\
IRAS 20340+5124  &166684&20 35 28.85&+51 35 27.4&Sc  &50.4&10.51& 1.62&3.41&2.89&32.2\\
UGC 11599        &65060 &20 36 33.82&+11 29 40.9&Sb  &67.2&10.37& 0.25&4.15&1.27&27.6\\
UGC 11723        &66579 &21 20 17.50&-01 41 03.5&Sb  &72.4&10.52& 0.77&3.74&2.25&29.8\\
NGC 7218         &68199 &22 10 11.71&-16 39 39.6&Sc  &23.7& 9.85& 0.13&3.44&2.16&33.0\\
MCG -04-52-024   &68313 &22 13 10.45&-22 26 42.2&Sab &75.6&10.40& 0.44&3.61&2.39&35.0\\
IRAS 22287+6137  &87389 &22 30 30.38&+61 52 49.9&Sc  &55.1&10.72& 2.75&3.51&2.89&34.8\\
NGC 7347         &69443 &22 39 56.16&+11 01 39.2&Sc  &34.3& 9.71& 0.46&3.43&2.06&31.0\\
NGC 7741         &72237 &23 43 54.37&+26 04 32.1&SBc &13.2& 9.19&-0.27&3.43&1.54&31.6\\
NGC 7755         &72444 &23 47 51.77&-30 31 19.5&Sc  &39.9&10.16& 0.02&3.71&1.93&29.6\\


==> 3881inp2.tex <==
MCG -02-02-005         &1404   &00 21 51.12&-09 29 32.0&S0-a&90.1&10.16&0.48&2.71&3.93&37.0\\
MCG -02-03-066         &3662   &01 01 19.43&-09 50 43.4&Sb  &65.3&10.22&0.65&2.59&4.23&40.4\\
IRAS F01222+0038       &5219   &01 24 48.93&+00 54 36.4&S0-a& 144&10.79&0.71&3.38&3.24&34.8\\
UGC 02403              &11075  &02 55 57.27&+00 41 33.0&SBa &53.8&10.68&1.15&2.49&4.89&38.3\\
IRAS F09489+2746       &139220 &09 51 46.50&+27 32 45.5&S?  & 147&10.63&1.08&3.29&3.24&36.0\\
MRK 0126               &28460  &09 52 36.83&+52 13 18.4&Sc  & 176&10.76&    &3.67&2.62&28.6\\
IRAS F10134+2230       &1666567&10 16 11.67&+22 15 35.3&S?  & 296&11.28&0.98&3.21&4.06&35.3\\
UGC 05605              &30393  &10 22 46.48&+48 38 13.7&Sb  & 225&10.96&0.48&3.12&3.92&32.3\\
MCG +08-21-055         &35717  &11 33 57.59&+45 16 00.0&Sab & 150&10.55&0.56&3.07&3.62&32.6\\
MCG +08-21-093         &36396  &11 43 04.49&+48 23 56.0&Sab &65.4&10.03&0.37&3.28&2.67&29.4\\
IRAS F12207+6329       &40158  &12 23 05.24&+63 13 21.2&S?  & 268&11.52&0.91&3.15&4.42&41.4\\
IC 3627                &139990 &12 39 32.02&+27 29 50.5&S?  & 257&11.07&1.02&3.29&3.69&37.5\\
UGC 08168              &45117  &13 03 41.11&+51 29 45.6&    & 178&10.77&    &3.13&3.72&34.0\\
NGC 5104               &46633  &13 21 23.11&+00 20 33.5&SBa &82.4&11.05&1.05&2.84&4.56&34.8\\
IRAS 13232+1731        &2816875&13 25 43.88&+17 15 53.0&S?  & 360&11.46&0.87&3.75&3.17&31.4\\
2MASX J13465224+1741550&48852  &13 46 52.24&+17 41 54.8&Sc  & 121&10.39&0.24&3.48&2.63&33.5\\
IRAS F13543+5846       &84079  &13 56 00.87&+58 31 47.3&    & 181&10.95&1.12&3.25&3.65&34.7\\
MCG +06-31-036         &49754  &13 58 41.85&+35 05 16.3&Sab & 157&11.26&1.20&3.15&4.16&34.7\\
UGC 08991              &50169  &14 04 35.96&+15 28 21.7&S?  & 117&10.31&0.22&3.14&3.22&36.5\\
NGC 5472               &50345  &14 06 55.03&-05 27 37.9&Sab &44.8& 9.88&0.57&2.83&3.42&32.5\\
2MASX J14080087+3613283&2077016&14 08 00.88&+36 13 28.3&S?  & 271&10.80&0.96&3.86&2.29&34.4\\
NGC 5520               &50728  &14 12 22.78&+50 20 54.4&Sb  &33.1& 9.86&0.14&2.97&3.11&31.3\\
IRAS F14105+0357       &50775  &14 13 06.91&+03 42 59.1&S?  & 114&10.61&0.81&3.24&3.33&35.0\\
IC 4405                &51167  &14 19 16.55&+26 17 54.8&Sab & 166&10.98&0.45&3.47&3.23&32.1\\
IRAS F14228+5351       &84158  &14 24 34.43&+53 38 23.9&S?  & 138&10.26&    &3.34&2.77&31.5\\
NGC 5637               &51736  &14 28 59.64&+23 11 29.5&Sc  &80.1&10.41&0.56&3.35&2.91&32.7\\
MCG +06-32-070         &52138  &14 35 18.42&+35 07 07.7&S?  & 129&11.07&    &3.60&3.07&34.8\\
IRAS F14490+5154       &52990  &14 50 41.24&+51 42 15.7&Sbc & 119&10.58&0.86&3.18&3.42&34.8\\
IRAS F14501+3823       &84327  &14 52 05.70&+38 10 59.4&S?  & 147&10.68&    &3.20&3.49&34.7\\
IRAS F15017+2417       &53766  &15 04 00.77&+24 06 17.6&    & 315&11.78&    &3.27&4.45&42.6\\
IRAS F15097-0248       &54279  &15 12 23.14&-02 59 57.9&S?  & 163&10.69&0.81&3.13&3.63&40.7\\
MCG +08-28-025         &55029  &15 24 51.04&+50 18 54.3&Sab & 170&10.66&0.54&3.39&3.08&30.2\\
IRAS F15305+4917       &84665  &15 32 07.80&+49 07 29.4&S?  & 114&10.73&    &3.23&3.48&33.7\\
IRAS 15313+5802        &55361  &15 32 31.70&+57 52 58.9&S?  & 182&10.84&0.44&3.22&3.61&40.0\\
IC 4581                &55893  &15 44 01.47&+28 16 36.9&Sc  & 151&10.65&0.43&3.11&3.63&37.1\\
UGC 10030              &56025  &15 47 00.41&-00 59 07.3&Sab & 133&10.66&0.50&3.15&3.56&30.1\\
IRAS F15538+5218       &56381  &15 55 10.89&+52 10 06.5&S?  & 169&10.88&0.48&3.61&2.87&35.2\\
MRK 1101               &56442  &15 56 36.42&+41 52 50.4&S?  & 157&11.03&0.65&3.24&3.75&36.3\\
IRAS 15557+4957        &2816987&15 57 14.00&+49 49 15.4&S?  & 191&10.75&0.76&3.11&3.74&36.3\\
MRK 0694               &56760  &16 02 01.78&+16 26 07.2&E-SO& 137&10.47&0.52&2.99&3.69&34.7\\
IRAS F16022+2008       &1613262&16 04 26.68&+20 00 32.5&S?  & 151&10.44&0.76&3.19&3.26&34.0\\
UGC 10325 NED01        &93134  &16 17 30.61&+46 05 30.4&Sb  &88.6&10.55&    &3.39&2.98&32.3\\
NGC 6113               &57807  &16 19 10.58&+14 08 01.1&S0-a& 134&10.77&0.39&3.51&2.96&29.5\\
NGC 6120               &57842  &16 19 48.10&+37 46 28.4&Sd  & 139&11.28&0.72&3.43&3.63&34.6\\
IRAS F16192+3958       &2156824&16 20 55.81&+39 51 39.7&S?  & 130&10.47&0.87&3.54&2.59&38.5\\
MCG +09-27-020         &57903  &16 21 17.74&+51 33 25.4&Sc  & 136&10.73&0.88&3.58&2.78&30.6\\
MCG +09-27-021         &57907  &16 21 25.86&+56 00 34.0&S?  & 136&10.57&0.78&3.20&3.36&30.5\\
MCG +08-30-009         &57940  &16 22 17.83&+50 22 19.0&Sb  & 259&11.45&0.89&3.15&4.36&35.4\\
MCG +07-34-018         &58046  &16 24 37.10&+39 07 40.0&Sb  & 158&11.04&    &2.97&4.30&35.2\\
NGC 6150B              &58100  &16 25 44.47&+40 28 32.4&Sab & 144&10.61&0.44&3.46&2.89&30.3\\
IRAS 16369+3721        &84761  &16 38 43.15&+37 15 18.0&S?  & 138&10.59&    &2.91&3.98&38.9\\
MCG +09-27-065         &58801  &16 42 04.48&+54 41 22.3&SBab& 143&10.63&0.86&2.97&3.89&39.4\\
NGC 6247               &59023  &16 48 20.25&+62 58 35.0&S?  &70.2&10.72&0.39&3.27&3.37&34.8\\
MCG +10-24-064         &59060  &16 49 27.83&+58 53 54.9&S?  &78.9&10.12&0.50&2.79&3.74&33.1\\
IRAS F16530+5033       &59232  &16 54 19.55&+50 28 30.6&S?  &47.4& 9.94&0.74&2.96&3.22&33.9\\
IRAS F17072+3627       &165719 &17 08 58.64&+36 23 56.7&S?  & 124&10.66&    &2.91&4.04&36.8\\
MCG +10-24-102         &59767  &17 11 00.57&+56 56 08.2&S?  & 132&10.57&0.47&3.53&2.71&35.1\\
IC 1249                &59919  &17 14 54.98&+35 31 14.2&S?  & 169&10.90&0.32&3.56&2.98&32.0\\
UGC 10812              &60074  &17 19 28.77&+40 55 22.7&SBb & 134&10.41&0.27&3.21&3.18&32.8\\
IRAS F17190+6219       &2633868&17 19 31.79&+62 16 47.3&S?  & 370&11.23&1.38&3.52&3.39&32.0\\
MCG +10-25-032         &60289  &17 26 25.86&+58 35 19.4&Sb  & 120&10.18&0.61&3.43&2.53&35.7\\
IRAS 17297+5127        &60428  &17 30 55.75&+51 25 50.4&S?  & 210&11.31&0.62&3.53&3.44&35.3\\
MCG +10-25-070         &60578  &17 36 57.54&+59 12 00.8&Sbc & 140&10.60&0.93&3.09&3.63&37.4\\
2MASX J21470265-0826288&1003693&21 47 02.67&-08 26 28.8&S?  & 276&11.06&1.07&3.18&3.91&34.8\\

